Enable people to identify science news based on retracted articles on social media

For many people, social media is an important way to consume news on important topics like health. Unfortunately, some influential health news is misinformation because it is based on retracted scientific work. Ours is the first work to explore how people can understand this form of misinformation and how an augmented social media interface can enable them to make use of information about retraction. We report a between subjects think-aloud study with 44 participants, where the experimental group used our augmented interface. Our results indicate that this helped them consider retraction when judging the credibility of news. Our key contributions are foundational insights for tackling the problem, revealing the interplay between people's understanding of scientific retraction, their prior beliefs about a topic, and the way they use a social media interface that provides access to retraction information.

==> 10_accessibility.tex <==
\section{\texorpdfstring{\centering{\Large{accessibility text of Figures and tables}}}{Lg}}

\subsection{Figures:}

\subsubsection{Figure~\ref{fig:teaser}:} The teaser figure under the title shows two Facebook style social media posts. Both of them follow the structure of social media interface. First there is the image of the post, then the source followed by Headline claim. The image on the left is a photo of a street where people are walking with masks on, while the left one is closeup shot of a surgical masks placed on a table. Both social media posts are coming from same news media source EMPR. The left posts has headline claim "Face masks most effective means to avert COVID-19 transmission" while the right post headline says" Surgical, Cotton Masks are Effective for Filtering SARS-Cov-2. 

\subsubsection{Figure~\ref{fig:study_flowchart}:} This figure shows the complete study flow overview which has been divided into four stages. In each stage participant go through some activities. Except stage S1, all stages have data collected from the activities carried out by participant. The figure has been described stage by stage in the text.

\subsubsection{Figure~\ref{fig:tutorial_reasons_retraction}:} This figure is a screenshot of the retraction tutorial that participant went through. It has a brief summary of what retraction in science publication context. It mentions that retraction due to research misconduct can invalidate scientific study claims. Next in the tutorial a list of reason for retraction are provided in red where participant can drag and drop each reason to one of the three groups. G1 indicates that the reasons added in it would invalidate the underlying article claim, G2 does not and G3 unsure. Each reason has more underlying details that are shown when participants hover on it. On figure the Fabrication underlying message is shown that says "Making up data or results rather than having them come from actual research, and recording or reporting them".

\subsubsection{Figure~\ref{fig:retraction_info_revealed}:} This figure shows the interface shown to Control and Treatment group. Social media interface A on the left was shown to control group and interface B was shown to participants in Treatment group. This figure has been thoroughly explained in text.

\subsubsection{Figure~\ref{fig:tutorial_retract_response}:} This figure shows list of participant P1 to P44 under their respective Control or Treatment group and their gender color coded as male-blue and female-pink. It also shows participant understanding of retraction and how they categorised each reason for retraction into the different groups. This figure has also been thoroughly described in text.

\subsubsection{Figure~\ref{fig:tutorial_fraudulent_reasons}:} This figure is the vertically aligned (rotated) and cropped version of Figure~\ref{fig:tutorial_retract_response}. The non-fraudulent reasons for retraction of Figure~\ref{fig:tutorial_retract_response} has been cropped out and the rest of is shown without any modification. The figure has been discussed in detail in the text.

\subsubsection{Figure~\ref{fig:tutorial_non-fraudulent_reasons}:} This figure is the vertically aligned (rotated) and cropped version of Figure~\ref{fig:tutorial_retract_response}. The fraudulent reasons for retraction of Figure~\ref{fig:tutorial_retract_response} has been cropped out and the rest of is shown without any modification. The figure has been discussed in detail in the text.

\subsubsection{Figure~\ref{fig:fig5}:} This is figure has two parts, part (a) is distribution of fraudulent reasons for retraction Fabrication, Falsification and Plagiarism into three groups G1,G2 and G3. Part (b) shows the  distribution of non-fraudulent reasons for retraction (Errors, Reproducibility, Permission and Duplicate publishing) into G1, G2 and G3. G1 means that retraction reason does not invalidate the scientific claim, G2 =  retraction reason does not invalidate the study claims while G3 =  retraction reasons grouped reasons for retraction into the three different group. Further details are available in text.

\subsubsection{Figure~\ref{pre_three_health_confidence}:} This figure shows three distinct distribution of participant confidence in their prior belief on a scale of 0 to 100 with increments of 10. Each for one health topic. First (a) is on \textit{Masks}, second sub figure is on \textit{Diet} and third is on \textit{Movie} health topic. All three distribution are progressively color coded. Shades of red to indicate confidence less than 50 percent, shades of green to indicate higher than 50 percent, and one shade of grey to indicate 50 percent. Further details for each distribution are provided with in text.



\subsubsection{Figure~\ref{fig:post_three_health_confidence}:} This figure shows three distinct distribution of participant confidence in their post belief on a scale of 0 to 100 with increments of 10. Each for one health topic. First (a) is on \textit{Masks}, second sub figure is on \textit{Diet} and third is on \textit{Movie} health topic. All three distribution are progressively color coded. Shades of red to indicate confidence less than 50 percent, shades of green to indicate higher than 50 percent, and one shade of grey to indicate 50 percent. Further details for each distribution are provided with in text.

\subsection{Tables:}

\subsubsection{Table~\ref{tab:pre_stance}:} This table shows the distribution of participant prior beliefs on three health topic using scale of Strongly agree, Somewhat disagree, Neither, Somewhat Agree and Strongly Agree. For each health topic mean and median are calculated and shown in the table. Further details about the exact distribution is discussed in text.





\subsubsection{Table}
